MABSplit: Faster Forest Training Using Multi-Armed Bandits

Random forests are some of the most widely used machine learning models today, especially in domains that necessitate interpretability. We present an algorithm that accelerates the training of random forests and other popular tree-based learning methods. At the core of our algorithm is a novel node-splitting subroutine, dubbed MABSplit, used to efficiently find split points when constructing decision trees. Our algorithm borrows techniques from the multi-armed bandit literature to judiciously determine how to allocate samples and computational power across candidate split points. We provide theoretical guarantees that MABSplit improves the sample complexity of each node split from linear to logarithmic in the number of data points. In some settings, MABSplit leads to 100x faster training (an 99% reduction in training time) without any decrease in generalization performance. We demonstrate similar speedups when MABSplit is used across a variety of forest-based variants, such as Extremely Random Forests and Random Patches. We also show our algorithm can be used in both classification and regression tasks. Finally, we show that MABSplit outperforms existing methods in generalization performance and feature importance calculations under a fixed computational budget. All of our experimental results are reproducible via a one-line script at https://github.com/ThrunGroup/FastForest.

==> 10-acknowledgements.tex <==
% !TEX root = 0-main.tex

\begin{ack}
\label{ack}
M. T. was funded by a J.P. Morgan AI Fellowship, a Stanford Indisciplinary Graduate Fellowship, a Stanford Data Science Scholarship, and an Oak Ridge Institute for Science and Engineering Fellowship.
\end{ack}


==> 11-futurework.tex <==
\section{Future Work \label{sec:futurework}}
\begin{itemize}
    \item faster hyperparameter search
    \item Can extend our approach to deal with missing data (as many RF do)
    We also demonstrated the use of \algname in common feature importance techniques for exploratory data analysis. Future work could compare such techniques to other techniques that have recently gained popularity, such as TreeShap \cite{lundberg2018treeshap} and FastTreeShap \cite{yang2021fasttreeshap}. \todo{[Have we done this?]}

Other potential future research directions include adaptively choosing features during feature subsampling, as well as developing a better understanding of the effect of \algname on the bias and variance of trained models.

A potential negative consequence of our work is that practitioners may be incentivized to gather and store larger amounts of data now that it can be meaningfully processed, in a phenomenon more generally described as induced demand \cite{induceddemand}. This incentive realignment could potentially result in negative externalities such as an increase in energy consumption and carbon footprints.
\end{itemize}
